Optimal Service Placement, Request Routing and CPU Sizing in Cooperative Mobile Edge Computing Networks for Delay-Sensitive Applications

We study joint optimization of service placement, request routing, and CPU sizing in a cooperative MEC system. The problem is considered from the perspective of the service provider (SP), which delivers heterogeneous MEC-enabled delay-sensitive services, and needs to pay for the used resources to the mobile network operators and the cloud provider, while earning revenue from the served requests. We formulate the problem of maximizing the SP's total profit subject to the computation, storage, and communication constraints of each edge node and end-to-end delay requirements of the services as a mixed-integer non-convex optimization problem, and prove it to be NP-hard. To tackle the challenges in solving the problem, we first introduce a design trade-off parameter for different delay requirements of each service, which maintains flexibility in prioritizing them, and transform the original optimization problem by the new delay constraints. Then, by exploiting a hidden convexity, we reformulate the delay constraints into an equivalent form. Next, to handle the challenge of the complicating (integer) variables, using primal decomposition, we decompose the problem into an equivalent form of master and inner sub-problems over the mixed and real variables, respectively. We then employ a cutting-plane approach for building up adequate representations of the extremal value of the inner problem as a function of the complicating variables and the set of values of the complicating variables for which the inner problem is feasible. Finally, we propose a solution strategy based on generalized Benders decomposition and prove its convergence to the optimal solution within a limited number of iterations. Extensive simulation results demonstrate that the proposed scheme significantly outperforms the existing mechanisms in terms of the SP's profit, cache hit ratio, running time, and end-to-end delay.

==> part3-temp.tex <==
%!!!\section{System Model and Problem Formulation}

%In this section, first we describe our system model... Later, we formulate the problem of joint service placement and routing in a cooperative MEC ...; a discussion of the problem time complexity follows. %The frequently used notation is summarized in Table~\ref{table:notation}.

\begin{table}[h!] 
\caption{Frequently Used Notations.}
\centering
\begin{tabular}{l p{0.7 \columnwidth} }
 Symbol & Description  \\ \hline
 % \multicolumn{2}{c}{Input Parameters} \\\hline
 $e \in \mathbb E$ & BS index\\ 
 $n \in \{\mathbb E, c\}$ & server  index\\ 
 $l_{en} \in \{0, 1\}$&indicates whether BS $e$ and server $n$ are connected \\
 $s \in \mathbb S$ & service index \\
 $C_e$ & storage limit at $\mathrm{BS}_e$ \\
 $B_e$ & communication limit at $\mathrm{BS}_e$\\
 $B^l_{en}$ & uplink/downlink communication limit at link $en$\\
 %$M_n$ & computation limit at server $n$ \\
 {{$M_e$}} & computation limit at $\mathrm{BS}_e$ \\
 $ d^{\text{prp}}_{en}$ & propagation delay of link $en$\\
 $\lambda_{es}$  & demand for service $s$ arrived at BS $e$ \\
 $\sigma_{s}$& size per replica of service $s$ \\
 $\beta_{s}$& size of input/output data per request of $s$\\
 $\nu_{s}$& average  computation complexity per request of $s$ \\
 $D^{\text{max}}_{s}$& target delay of service $s$ \\
 $r^{\textit{srv}}_{ns}$ & revenue gained by serving one request for $s$ at $n$\\
 $p^{\textit{cpu}}_{n}$& unit cost of computation at server $n$\\
  $p^{\textit{str}}_{n}$& unit cost of storage at server $n$\\
 $p^{\textit{trn}}_{en}$ & unit traffic cost at link $en$ \\\hline
 \multicolumn{2}{c}{Decision Variables} \\\hline
 $x_{ns} \in \{0, 1\}$ & placement variable of service $s$ at server $n$\\
 $y_{sen} \in [0,\,1]$ & delivering variable for the requests of service $s$ at BS $e$\\
 $u_{ns} \in \mathbb{R}^+ $& CPU size allocated to service $s$ at node $n$ \\\hline
  \multicolumn{2}{c}{Auxiliary Variables} \\\hline
$D^{\text{srv}}_{ns} \in \mathbb{R}^+$& average service delay of requests for service $s$ at server $n$ \\
$D^{\text{cng}}_{en} \in \mathbb{R}^+ $ & average congestion delay of link $en$\\
$\Lambda_{ns} \in \mathbb R^+$ & total requests for service $s$ delivered to server $n$\\
 $\Lambda^l_{en} \in \mathbb R^+$ & uplink/downlink traffic passing over link $en$\\ 
 $z_{sen} \in \{0, 1\}$& indicator variable for $y_{sen}$; 1 if $y_{sen}>0$ and $0$ otherwise\\\hline
\end{tabular}
\label{table1}
\end{table}

\section{System Model}\label{sec:model}
%{\color{red}{the relation of the MNO and MEC is not established well}}

In this paper, we study service placement, CPU sizing, and request admission and scheduling in a cooperative MEC system provided by one or possibly multiple mobile networks. This problem is modeled taking the perspective of a service provider (SP) which delivers MEC-enabled delay-sensitive services across these networks.
MNOs deliver edge-located computation and storage resources. These facilities are pre-installed and collocated with the operators' network, \eg, at BSs and aggregation sites  \cite{hu2015mobile}. 
%with communication capability.
SP should pay for used resources across the MEC network and the cloud to the MNOs and the cloud provider, respectively.  
%according to use over time
%specify the required capabilities across the MEC network and the cloud and
%\MA{changed:MEC does not include cloud.}

We consider a 2-tier network structure consisting of a remote cloud $c$ with abundant resources and a cooperative MEC system with a set of $E$ BSs, denoted by $\mathbb E=\{1,\cdots, E\}$,  distributed at fixed locations in a large service region, as illustrated in \figurename~\ref{fig:network}. Let $n \in \{\mathbb E, c\}$ be the index of a server %at the BSs or cloud.
(either a BS or the cloud). 
The BSs are connected to their neighboring BSs via low latency, high bandwidth LAN connection, and to the remote cloud via backhaul links. The existence of such a direct link between each $\mathrm{BS}_e$ and server $n$ is denoted by an indicator variable $l_{en}$, and  $B^l_{en}$ indicates the uplink/downlink bandwidth of the link. Here, all the BSs are assumed to be connected to the central remote cloud, and hence, we have $l_{ec}=1$ for all $e \in \mathbb E$.


%We consider a cooperative MEC system consisting of a remote cloud $c$ with abundant resources and a set of $E$ BSs, denoted by $\mathbb E=\{1,\cdots, E\}$,  distributed at fixed locations in a large service region, as illustrated in \figurename~\ref{fig:network}. The BSs can communicate with their neighboring BSs through low latency, high bandwidth LAN connection or V2X interfaces. The existence of such a link between each $\mathrm{BS}_e$ and $\mathrm{BS}_n, \forall e,n \in \mathbb E, $ is denoted by an indicator variable $l_{en}$, and  $B^l_{en}$ indicates the bandwidth of the link. Moreover, all the BSs are assumed to be connected to the central remote cloud through their backhaul links, and hence, we denote $l_{ec}=1$ for all $e \in \mathbb E$. 



Each $\mathrm{BS}_e$ is equipped with limited storage (hard disk), computation, and communication capacities indicated by $C_e$, $M_e$, and $B_e$, respectively. SP can lease storage and computation resources at server $n \in \{\mathbb E, c\}$ at unit costs $p^{\text{str}}_{n}$ and $p^{\text{cpu}}_n$, respectively. 
MNOs also charge SP at $p^{\text{trn}}_{en}$ per unit of bandwidth consumption between $\mathrm{BS}_e$ and server $n$. 
The computation cost at the cloud is typically cheaper than the  BSs. Furthormore, the aforementioned costs can also be different across different BSs depending on the location, owner MNO and its reputation, reliability, etc.    
%Moreover, the unit storage and computation costs at server $n \in \{\mathbb E, c\}$ are denoted by $p^{\text{str}}_{n}$ and $p^{\text{cpu}}_n$, respectively. 


%When a request for a service is arrived at any $\mathrm{BS}_e$, it can be served by the BS itself, or transferred to the neighbouring servers (either the cloud or the neighbouring BSs) to be served. In the latter case, the input/output data of the service needs to be communicated through the link between the BS and the target server, which occupies some communication bandwidth of the associated link. We denote by $ p^{\text{trn}}_{en}$ the unit transmission cost between $\mathrm{BS}_e$ and server $n$. 

%For the cloud, the aforementioned costs include/reflect the {\color{red}{leasing}} costs, while for the $\mathrm{BS}_n, \forall n \in \mathbb E$, 
%they enfold the leasing costs of a nearby edge cloud provider or the operational costs of the BS itself if the resources are owned by the mobile network operator (MNO) itself.}} 


The SP provides a library of $\mathbb S=\{1, \cdots, S\}$ latency-sensitive services, \eg, online gaming, autonomous driving, video streaming, which are heterogeneous in terms of storage, computation, and communication requirements \cite{huawei}. All BSs might receive requests for all the services and demand is assumed independent of service placements. We assume requests for each service $s$ arriving at $\mathrm{BS}_e$  
follow a Poisson process with average rate $\lambda_{es}$, which is a common assumption in existing works \cite{xu2018joint, ma2020cooperative}. Each service $s$ requires $\sigma_s$ storage units per replica to store its codebase and  required databases and its input/output data size per request is $\beta_s$ (wolog we assume the input and output data sizes per request are equal).
Furthermore, services can have different processing requirements depending on their computational complexity. The computational capability (in CPU cycles) required to process one request of service $s$ is assumed to be an exponential random variable with average $\nu_s$. 
Finally, services come from different applications with divergent delay requirements. For example, an online gaming service can tolerate less delay than a video streaming service.
We consider a target delay of $D^{\text{max}}_s$ for each service $s$, %as the most critical quality-of-service (QoS) metric 
which defines the maximum tolerable end-to-end delay for requests of service $s$. 
Table~\ref{table1} summarizes the list of all the frequently  used  notations.



\section{Problem formulation}\label{sec:problem}

Given the knowledge of the service request arrivals and MEC topology, the SP should decide about \begin{enumerate*}[label=\itshape\roman*\upshape)]
    \item service placement, \ie, which servers should run each type of service, \item workload admission and scheduling, \ie, which fraction of the received workload at each BS should be admitted and how it should be distributed across the neighboring BSs and the cloud, and \item CPU sizing, \ie, how much computation capacity should be allocated to each virtual machine for running its associated 
    service.
\end{enumerate*}
Following the previous works (\eg, see \cite{poularakis2020service}), we assume that the aforementioned  decisions are taken at the beginning of a long-time window during which the request rates are assumed to be fixed and predictable. In the following, we formalize these decisions, and introduce the objective function  and the system constraints in the problem of joint service placement, request admission and scheduling, and CPU sizing in a cooperative MEC system. 

\subsection{Decision  Variables and Constraints}

\textbf{Service Placement.}
Service placement is defined by the following matrix  
\begin{equation*}\label{eq:variable:x}
{\mathbf{X}} = [x_{ns} \in \{0, 1\}: n \in \{\mathbb E, c\}, s \in \mathbb S ],
\end{equation*}
where $x_{ns} = 1$ if service $s$ is stored in server $n$ and $x_{ns} = 0$ otherwise. Clearly, the total size of the  services placed on each $\mathrm{BS}_e$ should not exceed its storage capacity, \ie, 
\begin{equation}\label{eq:capacity:storage}
\sum_{s \in \mathbb{S}} \sigma_s x_{es} \leq C_e, \forall e.
\end{equation}


\textbf{Request Admission and Scheduling.}
%Upon receiving a request at a BS, SP needs to decide whether to admit it or not, depending on the latency and resources requirements of the service, and if it admits, to which server it should be delegated. 
For each service and each BS, the SP needs to decide which fraction of requests to admit, and how to schedule the admitted ones across servers, depending on the target delay of the service, its required resources, and leasing costs. Request scheduling allows each BS to delegate any fraction of arrived requests for a service to the cloud or any of its neighbouring BSs that have that service. This can help the servers to  efficiently and flexibly utilize the computational and storage capacity of the whole network. 
In order to formalize the request admission and scheduling, we define a service delegation matrix as 
\begin{equation*}\label{eq:variable:y}
{\mathbf{Y}} = [y_{sen} \in [0, 1]: s \in \mathbb S, e \in \mathbb E, n \in \{\mathbb E, c\}],
\end{equation*}
where $y_{sen}$ indicates the fraction of requests for service $s$ arrived at $\mathrm{BS}_e$ that are admitted and delegated to server $n$ for being served.

According to the above definition, clearly, at each $\mathrm{BS}_e$ and for each service $s$, we have the following normalization constraint over different associated delegation control variables, which indicates the sum of admitted requests cannot exceed $1$:
%, which indicates that for each service, the sum of the fractions of its requests at each BS that are delegated to other servers cannot exceed 1. 
\begin{equation}\label{eq:sum1}
\sum_{n \in \{\mathbb{E}, c\}} y_{sen} \leq 1, \forall s, e.
\end{equation}
Moreover, the communication capacity constraint of each $\mathrm{BS}_e$ should also be considered in the request admission, as follows
%Finally, we consider the communication capacity limit of each BS as
\begin{equation}\label{eq:capacity:bw}
\sum_{s \in \mathcal S}  \beta_s \sum_{n \in \{\mathbb E, c\}}  \lambda_{es} y_{sen} \leq B_e, \forall e.
\end{equation}
Finally, $\mathrm{BS}_e$ can delegate  requests for service $s$ to a server $n$ only if the service has been stored in that server and the server is  a neighbouring BS or the cloud, \ie,  
%Moreover, server $e$ can delegate  requests for service $s$ to a server $n$ only if the latter server is the cloud or a neighbour of the former server (there is a direct link between the two servers), i.e.,  
\begin{equation}\label{eq:routing}
y_{sen} \leq x_{ns} l_{en}, \forall s, e, n.
\end{equation}


\textbf{CPU Sizing.} Let matrix $\mathbf{U}$ represent the CPU sizing decision variable as 
\begin{equation*}\label{eq:variable:mu}
    {\mathbf{U}} = \{u_{ns} \in \mathbb R_+: n \in \{\mathbb E, c\}, s \in \mathbb S\},
\end{equation*}
where $u_{ns}$ represents the computation capacity (\eg, in GHz) reserved on server $n$ %to server requests 
for running service $s$. %At each BS, the computation capacity can be devoted to the placed services only, and such allocations should also preserve the BS's computation capacity constraint, {\color{red}{i.e., a feasible CPU sizing should satisfy the following two constraints}}
At each BS, the computation capacity allocations should preserve the BS's computation capacity constraint, \ie, a feasible CPU sizing should satisfy the following constraint
%{\color{red}{two constraints}} %\NA{ Constraint 5 is redundant because of constraint 6 and the fact that each $u_{es}$ is non-negative.} 
\begin{align}
    %u_{es}&\leq M_e, \forall s, e, \label{eq:p3:cons:sizing}\\
    \sum_{s \in \mathbb S} u_{es} &\leq M_e, \forall e.\label{eq:capacity:mu}
\end{align}
Note that the SP leverages virtualization technologies supported by the MEC system (\eg, virtual machine (VM), container, etc)  to deploy each service in isolation on the general-purpose server \cite{mecAndSlice}. This separation will ensure the safe operation, security, and privacy of running services, especially in terms of services with rigid QoS requirements or with access to customer information. 


\subsection{Delay Constraints} 

%In practice, most services belong to MEC applications with stringent delay requirements \cite{hu2015mobile}. 
%the maximum %service 
%delay that a service can tolerate is limited
%, known as maximum service delay 
%[ref?]. 
When a request for service $s \in \mathbb S$ is being served by server $n \in \{\mathbb E, c\}$, the end-to-end latency that it experiences should be less than the target delay of service $s$, \ie, $D^{\text{max}}_s$. 

The end-to-end latency that  a service request experiences includes three parts: 1) \textit{the propagation delay:} the round-trip propagation time of the direct link between the original BS at which the request has arrived and the destination server which is going to serve the request, 2) \textit{the congestion delay:} {\color{blue}{the total time it takes for the request and the response to be successfully  transmitted to the destination server and the original server, respectively, on the interconnecting link between the two servers, }} and 3) \textit{the service delay:} the processing delay at the destination server.  
Note that we only consider the network from BSs to the cloud, since the round-trip delay from users to the BS can be assumed to be fixed and small similar to other works \cite{yang2019cloudlet, nguyen2021two, ma2020cooperative}.  

More formally, we assume the dominant terms in the end-to-end latency for a service request originated at $\mathrm{BS}_e$ and  served at server $n$ are  the network delays of link $en$, and the service delay of service $s$ at server $n$. 
Let $D^{\text{srv}}_{ns}$ and $D^{\text{cng}}_{sen}$ denote the service delay of service $s$ at server $n$, and its congestion delay on link $en$, respectively, and $d^{\text{prp}}_{en}$ be the propagation delays of link $en$. 
Therefore, the target delay constraint can be represented as, 
\begin{equation}\label{eq:delay}
     (D^{\text{srv}}_{ns} + d^{\text{prp}}_{en} + D^{\text{cng}}_{sen}) \mathds{1}_{[y_{sen}>0]}  \leq D^{\text{max}}_s, \,\forall s, e , n, 
\end{equation}
where $\mathds{1}_{[y_{sen}>0]}$ is an indicator function which equals to $1$ only when $y_{sen}>0$. 


In the rest of this subsection, we derive the delay terms in the left hand side of the delay constraint in \eqref{eq:delay}. It should be noted that 
the propagation delay of all the network links are always fixed and can be assumed to be known, while the service and congestion delays highly depend on the admisison and scheduling policy. Therefore, it remains to derive the expressions of $D^{\text{srv}}_{ns} $ and $D^{\text{cng}}_{sen}$ as functions of the problem parameters and control variables. For this purpose, first note that as the arrival of requests for each service type $s$ at each $\mathrm{BS}_e $ is assumed to follow an independent Poisson process, with parameter denoted by $\lambda_{es}$,
the forwarded requests of service $s$ from any $\mathrm{BS}_e $ to a server $n$ is also a Poisson process with the new parameter $\lambda_{es}y_{sen}$, and hence,  the total requests for service $s$ served at server $n$ can also be modeled as a Poisson process with a rate of $\Lambda_{ns} = \sum_{e \in \mathbb E}\lambda_{es}y_{sen} $.
Similarly, the total uplink/downlink traffic over link $en$ between two BSs, \ie, for $n \in \mathbb E$, and over link $ec$ between a BS and cloud follows a Poisson process with rate $ \Lambda^l_{en} = \Lambda^l_{ne} = \sum_{s \in \mathbb S}\beta_s (\lambda_{es}y_{sen} + \lambda_{ns}y_{sne})$ and {\color{blue}{$\Lambda^l_{ec} = \Lambda^l_{ce}= \sum_{s \in \mathbb S}\beta_s \lambda_{es}y_{sec}$, respectively.}} 


From the definitions of $\nu_s$ and $ u_{ns}$, it follows that the processing time of each request for service $s$ at server $n$  is an exponentially-distributed random variable with the rate of $u_{ns}/\nu_s$. Therefore, the service delay of the requests for $s$ at server $n \in \{\mathbb E,c\}$ can be estimated by the average response time of an M/M/$1$ queue \cite{ross2014introduction} as
\begin{align}\label{eq: serving delay}
D^{\text{srv}}_{ns} =   \frac{1}{u_{ns}/\nu_s - \Lambda_{ns}}, \forall n, s.
\end{align}
Likewise, any link $en$ can be modeled as an M/M/1 queue with arrival rate of $\Lambda^l_{en}$ and service rate of  $B^l_{en}$. 
Consequently, the congestion delay at link $en$ is derived as 
\begin{align}\label{eq: congestion delay}
    D^{\text{cng}}_{sen} =   \frac{2\beta_s}{B^{l}_{en}-  \Lambda^l_{en}}, \forall s, e, n, n\neq e,
\end{align}
and $D^{\text{cng}}_{see} =0, \forall s, e$. Please observe that since network links and services are assumed to have symmetric uplink/downlink bandwidth and input/output size, respectively, the uplink and downlink congestion delay on link $en$ are equal, \ie, $D^{\text{cng}}_{en}=D^{\text{cng}}_{ne}$, and the round-trip congestion delay at link $en$ is two times of the congestion delay of uplink $en$ as shown above.
Finally, note that to ensure the stability of the aforementioned queues, we need the following two constraints: 
\begin{align}
    \Lambda_{ns} &\leq u_{ns}/\nu_s, \forall n,s, \label{eq:stability:node}\\
     \Lambda^l_{en} &\leq B^l_{en}, \forall e, n, n\neq e. \label{eq:stability:link}
\end{align}



\subsection{The Target/Formulated Optimization Problem}
We aim at maximizing the SP's total revenue gained from serving the services while minimizing the total cost of leased storage, computation, and communication resources. Services may belong to usecases with different latency, priority, and resource requirements. The SP will account for these differences while monetizing services. 


The SP's total serving revenue per unit of time can be expressed as
\begin{equation}\label{eq:revenue}
    \mathcal R_{\text{srv}} ({\bf{Y}}) = \sum_{s \in \mathbb S} \sum_{n \in \{\mathbb{E}, c\}}  R^{\textit{srv}}_{ns} \left(  \Lambda_{ns} \right), 
\end{equation}
where $R^{\textit{srv}}_{ns}$ is a twice continuously differentiable, 
concave and increasing function of the  total  requests  for service $s$ served at server $n$. Note that the above assumptions on the revenue function can capture a lot of interesting cases such as $\alpha$-fairness and proportional fairness \cite{omidvar2018optimal}. 


Moreover, the total cost includes the costs of leased storage, computation, and communication resources, which are described per unit of time, respectively, as:
\begin{align}
\mathcal P_{\text{str}}({\mathbf{X}}) &= \sum_{s \in \mathbb{S}} \sigma_s \sum_{n \in \{\mathbb{E}, c\}}  p^{\text{str}}_n  x_{ns},\label{eq:costs:str}\\
\mathcal P_{\textit{cpu}}({\mathbf{U}}) &= \sum_{s \in \mathbb{S}} \sum_{n  \in \{\mathbb E, c\}} p^{\textit{cpu}}_n   u_{ns},\label{eq:costs:cpu}\\
\mathcal P_{\text{trn}}({\mathbf{Y}}) &= \sum_{e \in \mathbb E}\sum_{n \in \{\mathbb E, c\}}  \Lambda^l_{en}p^{\textit{trn}}_{en}. \label{eq:costs:trn}
%\mathcal P_{\text{trn}}({\mathbf{Y}}) &= \sum_{s \in \mathbb S} \beta_s \sum_{e \in \mathbb E}\sum_{n \in \{\mathbb E, c\}} \lambda_{es} y_{sen} p^{\textit{trn}}_{en}\label{eq:costs:trn}.
\end{align}
Accordingly, the SP's total profit  %utility 
can be derived as %{\color{blue}{[wrote it separately for the purpose of saving space in the next equations.]}}
\begin{align}
    \mathcal{U}_{\text{total}} \left( \mathbf{X},\mathbf{Y},\mathbf{U} \right)
    =
    \mathcal R_{\text{srv}}({\mathbf{Y}}) - \mathcal P_{\text{str}}({\mathbf{X}}) -\mathcal P_{\text{cpu}}({\mathbf{U}}) -\mathcal P_{\text{trn}}({\mathbf{Y}}).
\end{align}
Finally, the problem of joint service placement, request admission and scheduling, and CPU sizing for the SP's profit maximization can be formulated as
%we write the optimization formulation as:
\begin{align}\label{eq:orig. opt.}
\mathcal{P}_{org}: \quad    &\max_{\mathbf{X,Y,U}} %\mathcal R({\mathbf{Y}}) - \mathcal P_{\text{str}}({\mathbf{X}}) -\mathcal P_{\text{cpu}}({\mathbf{U}}) -\mathcal P_{\text{trn}}({\mathbf{Y}})
\mathcal{U}_{\text{total}} \left( \mathbf{X}, \mathbf{Y},\mathbf{U} \right)
\notag\\
    &\text{subject to}\, \eqref{eq:capacity:storage}-\eqref{eq:stability:link}.
\end{align}

\subsection{Problem Complexity Analysis}
Problem $ \mathcal{P}_{org} $ includes both integer $\mathbf{X}$ and continuous ($\mathbf{Y}, \mathbf{U}$) variables, hence it is a mixed integer non-linear programming (MINLP) problem. In the following, we will describe a  simple instance of $\mathcal{P}_{org}$ and prove that it remains  NP-hard even in this simplified case. This will in turn prove that $ \mathcal{P}_{org}$ is NP-hard in the general form \eqref{eq:orig. opt.} and can not be solved in polynomial time.   
%In the following, we prove the NP-hardness of a special case which shows the problem can not be solved in polynomial-time in the general case.
%\blue{can be moved to Appendix from here and just keep theorem}


Consider a simple case where we do not take account of cost terms   \eqref{eq:costs:str}-\eqref{eq:costs:trn} in the objective function, \ie, all unit leasing costs $p^{str}_n$, $p^{\textit{cpu}}_{n}$, and $p^{\textit{trn}}_{en}$ are assumed to be $0$, and we consider linear and homogeneous revenue functions for each $s$, \ie, $R^{\textit{srv}}_{ns}=R^{\textit{srv}}_{s}=r^{\textit{srv}}_{s} \Lambda_{ns}, \forall n, s$. Setting capacities $B_e$, $M_e$, and $B^l_{en}$, $\forall e, n$, large enough eliminates constraints \eqref{eq:capacity:bw}, \eqref{eq:capacity:mu}, and  \eqref{eq:stability:link}, respectively, rules out decision variable matrix ${\mathbf{U}}$ and associated constraint \eqref{eq:stability:node}, and decrease delay terms $D^{\text{srv}}_{ns}$ and $D^{\text{cng}}_{sen}$ to zero in \eqref{eq:delay}. 
Moreover, we assume all BSs are connected by direct links with zero propagation delay, \ie, $l_{ee'} = 1$ and $d^{\text{prp}}_{ee'}=0, \forall e, e' \in \mathbb E$, and $d^{\text{prp}}_{ec} > \max_{s \in \mathbb S} {D^{\text{max}}_s}, \forall e$. 
%constraint \eqref{eq:delay} and ${\mathbf{Z}}$ variables can be ruled out since
Based on aforementioned assumptions,  \eqref{eq:delay} and \eqref{eq:routing} are satisfied for any $n \in \mathbb E$ and \eqref{eq:routing} is violated for $n=c$.
Therefore, in the optimal solution, no service will be placed on the cloud, and there is at most one instance for each service placed on all BSs, \ie,  $\sum_{e \in \mathbb E}{x_{es}} \leq 1$. If $x_{es}=1$, all request for that service will be delegated to $e$, \ie, $y_{se'e}=1, \forall e' \in \mathbb E$, and $y_{se'e}=0$ otherwise. Thus, we have $y_{se'e}=x_{es}, \forall e'$, and   
$\mathcal{P}_{org}$ can be rewritten as
\begin{align}
\mathcal{P}_{sp}: \quad&\max_{{\mathbf{X}} } \sum_{s \in \mathbb S} \sum_{e \in \mathbb{E}}  r^{\textit{srv}}_{s} x_{es} \sum_{e' \in \mathbb{E}} \lambda_{e's},\notag\\
\text{subject to}\, &\eqref{eq:capacity:storage}.\notag
\end{align}

\begin{theorem}[Problem Complexity]
Problem $\mathcal{P}_{\text{sp}}$ (which is a simple instance of $\mathcal{P}_{org}$) is NP-hard. 
\end{theorem}

\begin{proof}
We prove $\mathcal{P}_{\text{sp}}$ is NP-hard by reduction from the NP-hard 0-1 multiple knapsack problem (MKP)  defined as \cite{martello1990knapsack}: Given a set of $n$ items, where the weight of the $i$th item is $w_i$ and its profit is $v_i$, and a set of $m$ knapsacks ($m < n$), each having a maximum capacity $\hat{c}_j$, select $m$ disjoint subsets of items $\mathcal S_j$ such that the total profit of selected items, \ie, $\sum_{j=1}^{m} \sum_{i \in \mathcal S_j}v_i$, is maximum, and each subset $S_j$ can be assigned to a different knapsack $j$ whose capacity is not less than the weight of all items in the subset, \ie, $\sum_{i \in \mathcal S_j}w_i \leq c_j$. 

For an instance of MKP($[v_i]$, $[w_i]$, $[\hat c_j]$), we construct an instance for the special case of $\mathcal{P}_{\text{sp}}$ as follows: we associate each item $i$ to service  $s_i$ with $v_i=\sum_{e \in \mathbb{E}} \lambda_{es_i}$ and $w_i=\sigma_{s_i}$. For each knapsack $j$, we also consider a $\mathrm{BS}_j$ with $C_j=\hat c_j$.  
Let ${\mathbf{X}}$ be the optimal solution to $\mathcal{P}_{\text{sp}}$ and $\mathcal S_j=\{i \in \{1, \cdots, n\}: x_{js_i}=1\}$ be the set of all placed services on $\mathrm{BS}_j$. Since optimal solution will place each service on at most one BS and will preserve constraint \eqref{eq:capacity:storage}, it is easy to see that ${\mathbf{X}}$ is the optimal solution to $\mathcal{P}_{\text{sp}}$ if and only if $S_j$ ($j=1,\cdots,m$) is the optimal solution of MKP. 
\end{proof}
\blue{we may change the location of this subsection to a better place, maybe to the next section, or just put it as a remark}


==> part4.tex <==
\red{!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!}
\section{Solution Strategy}\label{sec:solution}
%naeimeh
As mentioned in the previous section, the formulated problem is an MINLP, where the coupling between the integer %variables $\mathbf{X}$ 
and continuous variables complicates the problem. 
%\blue{
Moreover, due to %the  non-linear terms in 
the constraints of the form \eqref{eq:delay}, %*** which include the product of continuous-continuous %and \red{continuous-integer} variables, 
even relaxing the integer variables cannot help to address this problem in polynomial time, as the relaxed version of the problem still remains non-convex.
%\NA{[Remove it?] :}  
Consequently, the conventional mixed-integer linear programming (MILP) or convex programming approaches cannot handle this problem.   

To overcome the aforementioned challenges efficiently, we introduce a new design trade-off parameter for different delay requirements of each service, providing flexibility in prioritizing different service delay requirements. 
By exploiting a hidden convexity, we reformulate the delay constraints into an equivalent form. Next, to handle the complicating integer variables, we use primal decomposition, decomposing the problem into an equivalent master and inner problems, over   complicating and simple variables, respectively. We employ a cutting-plane approach to build adequate representations of the extremal value of the inner problem as a function of the complicating integer variables and the set of values of the integer variables for which the inner problem is feasible.

\iffalse 
%*To tackle the challenges in solving the problem, we first introduce a design parameter for different delay requirements of each service, which maintains a trade-off between the priority of satisfying different service delay requirements. 
Then, by exploiting a hidden convexity, we reformulate the delay constraints into an equivalent form. 
%**To tackle the challenges in solving the problem, we first introduce a design trade-off parameter for different delay requirements of each service, and then exploit a hidden convexity to reformulate the delay constraints. 
%*By introducing a design trade-off parameter for various delay requirements of each service and then exploiting a hidden convexity, we reformulate the problem into a 
Next, to handle the challenge of the complicating integer variables, using primal decomposition, we decompose the problem into an equivalent form of master and inner problems, containing only complicating and simple variables, respectively. %disjointing the complicating and simpel variables.
We then employ a cutting-plane approach for building up adequate representations of the extremal value of the inner problem as a function of the complicating/integer variables and the set of values of the complicating/integer variables for which the inner problem is feasible. 
\fi

Finally, we propose a solution strategy based on generalized Benders decomposition (GBD) and prove its convergence to the optimal solution within a limited number of iterations. Before that, we will briefly review the GBD approach in the next subsection.

\iffalse
To solve this problem, 
in the rest of this section, 
we propose a solution strategy based on generalized Benders decomposition (GBD) \cite{geoffrion1972generalized} and prove its global convergence to the optimal solution of $\mathcal P_{org}$.   
%which has provable convergence to the global solution of $\mathcal P_{org}$.   
%to handle the complicating integer variables efficiently. 
Before that, we will briefly review the GBD approach in the next subsection. 
\fi

\subsection{Generalized Benders Decomposition}
Generalized Benders decomposition \cite{geoffrion1972generalized}, %proposed by Geoffrion as 
an extension to the vanilla Benders decomposition \cite{bnnobrs1962partitioning}, has been mainly used for solving a class of  MINLP problems of the form  
%GBD, proposed by Geoffrion \cite{}, is a generalization of Benders' approach \cite{} to a class of problems of the form 
\begin{equation}\label{eq: org GBD opt prob}
    \max_{\mathbf{x},\mathbf{y}} \{f(\mathbf{x},\mathbf{y}); ~ G(\mathbf{x},\mathbf{y}) \geq 0, \mathbf{x} \in \mathcal X, \mathbf{y} \in \mathcal Y\},
\end{equation}
%where $\mathbf{x}$ and $\mathbf{y}$ are vectors of variables, $G(\mathbf{x},\mathbf{y})$ is a vector of inequality constraints, and $y$ is a vector of integer variables, the so-called \textit{complicating} variables. By complicating, it means that when $y$ is fixed to some feasible value, the remaining problem is easy to solve. 
where $\mathbf{y}$ is a vector of \textit{complicating variables} in the sense that the above optimization is much easier to solve with respect to $\mathbf{x}$ when $\mathbf{y}$ is temporarily held fixed, and  $G(\mathbf{x},\mathbf{y})$ is a vector of constraint functions defined on $\mathcal X \times \mathcal Y $. 
The GBD approach decomposes the above problem into two simpler sub-problems, named {\textit{inner}} and \textit{outer}, and iteratively solves these two sub-problems in a way that obtains the optimal solution.  
%Under the GBD approach, the original problem is decomposed into two simpler problems, {\textit{inner}} and \textit{outer} and then the optimal solution is obtained by iterating between these two sub-problems. 
The inner problem is simply the original problem for some fixed values of $\hat{\mathbf{y}} \in \mathcal Y$:
\begin{equation}
    \max_{\mathbf{x} \in \mathcal X} f \left( \mathbf{x} , \hat{\mathbf{y}} )\,\, \text{subject to}\,\, G( \mathbf{x}, \hat{\mathbf{y}} \right) \geq 0,  
\end{equation}
and the outer problem, a.k.a. the master problem, is defined as 
%The derivation of master problem  features both inner and outer optimizations as:
\begin{align}
    &\max_{\mathbf{y}} v(\mathbf{y}) \\
    \text{subject to}\,\, &v(\mathbf{y}) = \{\sup_{\mathbf{x} \in \mathcal X} f\left( \mathbf{x} , \mathbf{y} \right); G\left( \mathbf{x}, \mathbf{y} \right) \geq 0 \},\notag\\
    & \mathbf{y} \in \mathcal Y \cap V,\notag
\end{align}
where $V\triangleq \{y: G\left( \mathbf{x}, \mathbf{y} \right)  \geq 0\, ~ \text{for some}\, \mathbf{x} \in \mathcal X \}$, includes the set of complicating variables for which there is a feasible solution to the original problem. 
%where $V\triangleq \{y: g(x, y) \geq 0\, \text{for some}\, x \in \mathcal X\}$, include the set of complicating variables for which there is a feasible solution.

Note that due to the primal decomposition, the above decomposition is optimal and the master problem is equivalent to the original problem in \eqref{eq: org GBD opt prob}  \cite{palomar2006tutorial}, \cite{bertsekas1997nonlinear}. However, 
the  function $v(y)$ and the set $V$ in the definition of the master problem are only known implicitly via their definitions. To deal with this difficulty, the dual representations of $v$ and $V$ and the relaxed version of the master problem are adopted %to provide 
which result in the following problem formulation:
\begin{subequations}\label{eq: relaxed master prob}
\begin{align}
    & \max_{ y_0, \mathbf{y} }  y_0  \tag{\ref{eq: relaxed master prob}}\ \\
    \text{subject to}& \notag \\
    & y_0 \leq L^\ast \left( \mathbf{y} ; \mathbf{\mu}^j \right) , ~ \forall j \in \left\{ 1,\ldots,\tau^{\text{feas}} \right\} , \label{eq: feas const} \\ 
    & L_\ast \left(\mathbf{y}; \lambda ^j \right) \geq 0, ~ \forall j \in \left\{1,\ldots,\tau^{\text{infeas}} \right\}, \label{eq: infeas const}
\end{align}
\end{subequations}
where Lagrange functions $L^\ast \left(\mathbf{y}; \mathbf{\mu} \right)$ and $L_\ast \left( \mathbf{y}; \mathbf{\lambda}  \right)$ are defined as 
%\MA{can change to $\mu$ and $\lambda$ similar to the next section}
\begin{align} \label{eq: L11}
 L^\ast \left(\mathbf{y}; \mathbf{\mu} \right) \triangleq \sup_{x \in \mathcal X}  \left\{ f  \left(\mathbf{x}, \mathbf{y} \right) + {\mathbf{\mu}}^T \mathbf{G} \left( \mathbf{x},  \mathbf{y} \right)  \right\},
\end{align}
and
\begin{align} \label{eq: L21}
    &L_\ast \left( \mathbf{y}; \mathbf{\lambda}  \right) \triangleq \sup_{ \mathbf{x} \in \mathcal X}  \left\{  {\mathbf{\lambda}}^T \mathbf{G} \left( \mathbf{x} , \mathbf{y} \right)  \right\},\\
    &\text{subject to}\quad \mathbf{1}^T \mathbf{ \lambda} = 1\notag,
\end{align} 
and $\mu^j$ and $\lambda^j$ are the %{\color{red}{optimal}}
Lagrangian multiplier vectors  of the  constraints in $G \left( \mathbf{x}, \mathbf{y} \right)$, in the $j^{\text{th}}$ feasible or infeasible iteration of 
 the inner problem, respectively. Moreover,  $\tau^{\text{feas}}$ and $\tau^{\text{infeas}}$ are the counters for %indicate 
 the number of feasible and infeasible iterations, respectively.  
 %is feasible or  \red{infeasible at the $\mathrm{j}^{th}$ iteration, respectively}. 
%and $u^j$ and $\lambda^j$ are Lagrange multipliers of the  constraints in $G(x, y)$ in the  feasible inner and \blue{infeasible inner problems} at iteration $j$, respectively. 
As such, at each iteration, one constraint of the form of \eqref{eq: feas const} (\textit{optimality cut}) or  \eqref{eq: infeas const} (\textit{feasibility cut}) will be added to the constraints  of  the  relaxed  master  problem, and $\tau^{\text{feas}}$ or $\tau^{\text{infeas}}$ will be incremented by one,
 depending whether the inner problem is feasible or infeasible. %but still not optimal. % the current solution is still
In this way, at each iteration, the GBD algorithm constructs a relaxed master problem which maintains an upper-bound to the solution of the original problem. On the other hand, note that the inner problem basically  maintains a lower-bound to the solution. The algorithm then %!!!proceeds in a way that reduces 
iteratively proceeds to reduce the gap between these two bounds, until it becomes small enough and hence, the convergence to the optimal solution is obtained. As proved by Geoffrion \cite{geoffrion1972generalized}, under some %sufficient
proper conditions, the GBD algorithm terminates in a finite number of iterations, converging to the global optimal solution of the original MINLP problem. 

%\NA{Will merge the following sentence with the above paragraph, properly: } 
%Note  that  constraints  (20a)  and  (20b)  define  \textit{optimality cut} and  \textit{feasibility cut}, respectively, which will be added to the constraints  of  the  relaxed  master  problem  by  the  algorithm, when required/applicable.

\begin{remark}\label{rem: convexity of the inner prob}
%A necessary condition to 
To ensure the  convergence of the above iterative method to the global optimal solution, %is that 
the inner problem %should
is required to be convex \cite{geoffrion1972generalized}. 
%\NA{I will write it later on (and maybe in a separate subsection) [It is good here for now].}
\end{remark}

\begin{remark} 
It should be noted that solving the relaxed master problem in \eqref{eq: relaxed master prob} is still challenging. This is mainly due to the fact that obtaining the Lagrange functions still involves optimization over both simple and complicating variables (i.e., the same  challenge we had with the original problem). To tackle this challenge, Geoffrion proposes some sufficient conditions, named \textit{Property P} \cite{geoffrion1972generalized}, on the original problem which help %!!! allows the involved supremums over $\mathcal X$ to be taken  independently of $\mathbf{Y}$, and hence, an
to obtain an explicit form for the Lagrange functions in \eqref{eq: L11} and \eqref{eq: L21}, resulting in bypassing the involved  optimization problems. Property P  allows  the involved  supremum over $\mathcal X$ to be taken  independently of $\mathbf{y}$.
%The outer problem is still difficult to solve in its current form since it involves inner optimization problems. To obtain the Lagrange functions for the master problem in explicit form, Geoffrion stated a property (P) which allows the supremum over $\mathcal X$ to be taken  independently of $y$. 
One important class of problems in which this property holds is the case where the functions $f$ and $G$ are linearly separable in $\mathbf{x}$ and $\mathbf{y}$ \cite{floudas1995nonlinear}.% \cite{geoffrion1972generalized}. %\NA{I want to revise it later.}
\end{remark}



Considering the illustrated iterative GBD method and the aforementioned remarks, in the following, we will first  investigate the potential of utilizing the GBD approach to our optimization problem $\mathcal{P}_{org}$ and then introduce our proposed  GBD-based algorithm to solve it.  % considering the above remarks.

\subsection{Problem Reformulation}\label{sec:solution:reformulate}

First note that in our problem formulation $\mathcal P_{org}$, the integer variables in $\mathbf{X}$ are the complicating variables. Therefore and according to Remark \ref{rem: convexity of the inner prob}, to ensure the global convergence of the GBD approach, it is necessary to prove that for any fixed values of %the complicating variables 
$\mathbf{X}$, the formulated problem is convex. %!!! [We will have the following commented part, if we keep the variable Z], as stated in the following lemma.
%
\iffalse %!!!

%To apply GBD on $\mathcal P_{org}$, we take $\mathbf{(X, Z)}$ as complicating variables. Under this assumption, we need this preliminary result,
\begin{lemma}\label{lem:convex}
    For any fixed values of the  integer variables $\mathbf{(X, Z)}$, $\mathcal P_{org}$ is convex in $\mathbf{(Y, U)}$.
\end{lemma}
\begin{proof}
    First note that clearly, the objective function and all the constraints except \eqref{eq:delay} are affine. Hence, it remains to prove that constraint \eqref{eq:delay} is convex, which is easy to verify when $\mathbf{Z}$ is fixed, %For this purpose, we note that when $\mathbf{Z}$ is fixed, this constraint is convex 
    due to the convexity of the terms in \eqref{eq: serving delay} and \eqref{eq: congestion delay}.
\end{proof}
\fi
%
For this purpose, first note that  the objective function $\mathcal{U}_{\text{total}} \left( \mathbf{X}, \mathbf{Y},\mathbf{U} \right)$ is concave, and all the constraints %in $\mathcal{P}_{org}$, except 
but constraint  \eqref{eq:delay} are affine. Hence, it remains to prove that the delay constraint stated by \eqref{eq:delay} is convex. However, constraint \eqref{eq:delay} involves  non-convex indicator functions. %In addition, this constraint includes the multiplication of the binary and the continuous variables, which
Moreover, because of  its  non-convexity, this constraint is not linearly separable in $\mathbf{y}$, and hence,  the optimization problem lacks property P, too. As such, the relaxed master problem still remains MINLP,
%. Therefore, due to the aforementioned challenges, 
and the formulated problem,  $\mathcal P_{org}$, cannot benefit from the GBD approach in its current form. 

%!!!! 
%\NA{New version: (will comment the old version below, at the end)}

%To tackle the aforementioned challenges, we first convert the delay constraint to a more conservative form

%\NA{old version: }
To tackle the aforementioned challenges,
%However, we have the product of variables in the joint binary-continuous domain in constraint \eqref{eq:delay} which threatens the applicability of GBD according to Remark~1 since the outer problem still remains MINLP. To handle this problem, 
we introduce the following relaxation to constraint \eqref{eq:delay}, which transforms its current formulation %the current formulation of \eqref{eq:delay}
to a linearly separable form such that the inner problem still remains convex and also property P preserves. Let $(1-\alpha) D^{\text{max}}_s$ and $\alpha D^{\text{max}}_s$ for $\alpha \in [0, 1]$ denote the maximum tolerable service  delay, and congestion and propagation delays, respectively, i.e., 
\begin{align}
       D^{\text{srv}}_{ns} \mathds{1}_{[y_{sen} > 0]} & \leq  D^{\text{max}}_s, \, \forall s, e, n=e,\notag\\
       D^{\text{srv}}_{ns}  \mathds{1}_{[y_{sen} > 0]} &\leq \left( 1- \alpha \right) D^{\text{max}}_s, \,\forall s, n \neq e, \notag\\
       (D^{\text{cng}}_{sen} + d^{\text{prp}}_{en}) \mathds{1}_{[y_{sen} > 0]} &\leq \alpha D^{\text{max}}_s, \forall s, e, n \neq e, \notag
\end{align}
where the first inequality %is for the case when 
is the delay constraint for the case when the request is served at its original BS, i.e., the request encounters only a  service delay at its serving BS, but  %there is 
no network delay. 
Note that summing up the above delay constraints results in the previous constraint \eqref{eq:delay}, however, the above form of delay constraints provides a  more flexible design than that of our originally formulated delay constraint. \red{This is due to the fact that  parameter  $\alpha$ maintains a design trade-off 
between the priority of satisfying %the
different service requirements.} % for the SP. % and \red{???}.
%!!!! MA: Note that the $\alpha$ parameter represents the importance of satisfying services for the SP. 
In more details, {\color{blue}{[NA: need to revise this part together] when $\alpha$ is set to a large value,  the SP allows to serve a request even if it has to go through a relatively saturated link (i.e., with high network delay) which in turn tightens the delay bound for service delay and increases the required computational resources.}} Later in Sec.~\ref{sec:evaluation}, \blue{we will discuss more on how different values of $\alpha$ can impact the solution strategy.} 


%!!!! Note that the above set of delay constraints are still non-convex.  Therefore, to tackle this challenge, we first define a new auxiliary variable 


%!!!! Although the above set of delay constraints are still non-convex, they  can  be reformulated as the following form, where all the constraints are now linear: 

Although the above set of delay constraints are still non-convex, in the following, we reformulate them in an equivalent form where all the constraints are now linear. For this purpose, we first define a matrix of  auxiliary binary variables $ \mathbf{Z} = [ z_{sen} \in \{ 0,1\}:  s \in \mathbb{S} , e \in \mathbb{E}, n \in \left\{ \mathbb{E}, c \right\} ] $ in which the element $z_{sen}$ indicates %whether any request for service $s$ originated on $\mathrm{BS}_e$ is transferred to server $n$. 
whether any request for service $ s $ originating at BS $ e $ is transferred to server $ n $  %indicator variable for $y_{sen}$ 
 (i.e, $ z_{sen} = \mathds{1} [y_{sen}>0] $). 
Therefore, the above set of constraints can be %equivalently
replaced with  
%\begin{subequations}\label{eq:const:delay2}
\begin{align}\label{eq:const:delay2_a}
    z_{sen}%&
    \leq D^{\text{max}}_s (u_{ns}/\nu_s - \Lambda_{ns}), \,\forall s, e, n=e,%\\
\end{align}
\begin{align}\label{eq:const:delay2_b}
    z_{sen}%&
    \leq (1-\alpha) D^{\text{max}}_s (u_{ns}/\nu_s - \Lambda_{ns}), \,\forall s, e, n\neq e,%\\
\end{align}
\begin{align}\label{eq:const:delay2_c}
    z_{sen}%&
    \leq \max \{(\alpha D^{\text{max}}_s - d^{\text{prp}}_{en}), 0\} (B^l_{en} - \Lambda^l_{en}),\, \forall s, e, n \neq e,
    %y_{sen} &\leq (\alpha D^{\text{max}}_s - d^{\text{prp}}_{en}),\, \forall s, e, n \neq e, 
\end{align}
%\end{subequations}
\begin{equation}\label{eq:const:delay2_d}
    y_{sen} \leq z_{sen}, ~ \forall s,e,n, 
\end{equation}
%!!!!where $z_{sen}$ is a binary variable indicating whether any request for service $s$ originated on $\mathrm{BS}_e$ is transferred to server $n$,  and hence, we should have the following additional  constraint 
%\begin{equation}\label{eq:variable:z}
%     y_{sen}  \leq z_{sen}, \forall s, e, n, 
%\end{equation}
%!!!!
where inequality \eqref{eq:const:delay2_c}  %enforces
is to ensure that $y_{sen}=0$ when $\alpha D^{\text{max}}_s < d^{\text{prp}}_{en}$. Note that this happens when the parameter $\alpha$ is set to a very small value or the associated service is so delay-sensitive that no network delay is tolerable for serving the requests, and hence, no service request can be delegated from its original BS to another server.  
%Note that the $\alpha$ parameter represents the importance of satisfying services for the SP. When $\alpha$ is large, the SP allows to satisfy a request even though it has to go through a saturated link with high network delay which in turn tights the delay bound for service delay and increases the required computational resources. In Sec.~\ref{sec:evaluation}, we discuss how different values of $\alpha$ can impact the solution.  
Moreover,    inequality \eqref{eq:const:delay2_d} is to  guarantee that no portion of the requests for service $s$ arrived at $\mathrm{BS}_e$ can be served by server $n$ if  it is not transferred to that server. 

Finally, we note that with constraint  \eqref{eq:const:delay2_d}, we can equivalently replace constraint \eqref{eq:routing}, which includes both complicating and simple variables,  with the following constraint that includes the complicating variables only:
\begin{align}\label{eq:const:delay2_e}
    z_{sen} \leq x_{ns} l_{en},~\forall s,e,n.
\end{align}
%Note to ourselves: This   constraint \eqref{eq:const:delay2_e} is added to reduce the solution space of the outer problem which helps us in the simulations.

\begin{remark}
    We note that an alternative way to handle %multiplication of terms 
    the non-convexity issue of the indicator term 
    in the on-off constraint \eqref{eq:delay} is to model the indicator function $\mathds{1}_{[y_{sen} > 0]}$ by using a big-M approach \cite{williams2013model} which makes the constraint linear in terms of the $y_{sen}$ variables. 
    %binary variable.
    However, this method imposes some new  computational difficulties as well as numerical issues in practical implementations, %{\color{blue}{[Check with MA] as this method adds two new decision variables to the master problem for which the inner problem may be infeasible}}, and also  
    since parameter $M$ needs to be carefully set in practice, to prevent %possible/
    numerical  instability issues.
    
%    Beside computational difficulties, this method adds new parameter $M$ which also needs to be properly set. Besides, the current formulation provides feasible solutions for each value of binary variables, while using big-M approach, two decision variables should be set in the master problem for which the inner problem may be infeasible. \MA{can be moved to the end of next sebsection.}
\end{remark}

% \blue{Now, considering the 
% new form of the delay constraints as stated in \eqref{eq:const:delay2_a}-\eqref{eq:const:delay2_d}, the formulated optimization problem  preserves both convexity of the inner problem and Property P. Consequently, [MA:remove? Already clarified in the next subsection]} we can utilize the GBD approach for solving it efficiently, which will be presented in the rest of this section.

Now, considering the new form of the delay constraints as stated in \eqref{eq:const:delay2_a}-\eqref{eq:const:delay2_d}, we can utilize the GBD approach to solve our problem efficiently, which will be presented in the rest of this section.


\subsection{The Proposed GBD-Based Solution Strategy}\label{sec:solution:GBD}
%\subsection{GBD-based Approach}\label{sec:solution:GBD}

%!!!For convenience, we first define the joint domain of service delegation and CPU sizing decision variables as

%The target optimization problem can be written as
For convenience, we first  write the  target optimization problem as 
\begin{subequations}\label{eq: Porg_reformed}
\begin{align} 
 \mathcal P_{org}^{\text{reformulated}} : ~ &\max_{ \mathbf{X} , \mathbf{Z} }
\max_{ \mathbf{Y}  ,  \mathbf{U} } ~ \mathcal{U}_{\text{total}} \left( \mathbf{X}  ,\mathbf{Y},\mathbf{U} \right) \tag{\ref{eq: Porg_reformed}} \\
    \text{subject to} \,\, ~
    &\eqref{eq:capacity:storage}, \eqref{eq:const:delay2_e}, \\
    %&z_{sen} \leq x_{ns} l_{en},~\forall s,e,n,\label{eq:const:delay2_e}\\
    &\mathbf{G} \left( \mathbf{X} , \mathbf{Z} ,\mathbf{Y},\mathbf{U} \right) \geq \mathbf{0}, \\
    &\left( \mathbf{X} , \mathbf{Z} \right) \in D_{X,Z},\\
    & \left( \mathbf{Y} ,  \mathbf{U} \right) \in \mathcal D_{Y,U},
\end{align}
\end{subequations}
where the binary elements of matrices  $\mathbf{X}$ and $\mathbf{Z}$ are the complicating variables. Moreover, $D_{X,Z} \triangleq \{0,1\}^{(E+1)\times S} \times \{0,1\}^{S \times E \times  (E+1)}$ defines the joint domain of service placement and auxiliary request transfer decision variables, and $D_{Y,U} \triangleq 
    [0,1]^{ S \times E \times (E+1) } \times \mathbb R_+^{(E+1) \times S}$ defines the joint domain of request scheduling and CPU sizing decision variables.   
    Finally,  $\mathbf{G} \left( \mathbf{X} , \mathbf{Z},\mathbf{Y},\mathbf{U} \right)$ is %{\color{blue}{an XXX-vector}} 
the vector of constraint functions defined on  $
%\{0,1\}^{(E+1)\times S} 
D_{X,Z} \times \mathcal D_{Y, U}$ and  determined by all the constraints that include the simple variables% only or the constraints that include both the simple and complicating variables
, i.e., constraints \eqref{eq:sum1}, \eqref{eq:capacity:bw}, \eqref{eq:capacity:mu}, \eqref{eq:stability:node}, \eqref{eq:stability:link}, 
and \eqref{eq:const:delay2_a}--\eqref{eq:const:delay2_d}. 

%\eqref{eq:routing} and \eqref{eq:p3:cons:sizing}, i.e. $\mathbf{G} \left( \mathbf{X},\mathbf{Z},\mathbf{Y},\mathbf{U} \right)=[y_{sen} \leq l_{en} x_{ns},\, \forall s, e, n;\, u_{es} \leq M_e x_{es},\, \forall e, s]$.%, and \eqref{eq:delay}. 

%!!!Now, considering the above formulation, the inner and outer problems defined in the GBD method can be derived as 
Considering the above formulation, we next proceed to obtain the inner and outer problems that will be used in our GBD-based solution strategy. % For this purpose,
%we first define the set of  
%\begin{align}
%    V = 
%\end{align}
%where 
%The set V consists of those values of y for which (l-y) is feasible; Y n V can be thought of as the projection of the feasible region of (1) onto y-space.
Note that the 
The inner problem can be derived as, %$ \forall \left( \hat{\mathbf{X}}, \hat{\mathbf{Z}} \right) \in \mathcal D_{X,Z} $, 
\begin{align}  \label{eq: P_in}
\mathcal{P}_{in}:
\quad f \left( \hat{\mathbf{X}} , \hat{\mathbf{Z}}  \right) \equiv &\max_{ (\mathbf{Y} , \mathbf{U}) \in \mathcal D_{Y,U} } ~ \mathcal R_{\text{srv}}({\mathbf{Y}}) - \mathcal P_{\text{cpu}}({\mathbf{U}}) -\mathcal P_{\text{trn}}({\mathbf{Y}})\notag \\
    &\text{subject to}\,\, ~ \mathbf{G} \left( \mathbf{\hat X}, \hat{\mathbf{Z}} , \mathbf{Y},\mathbf{U} \right) \geq \mathbf{0}, %, \notag \\
    %&\hspace{42 pt} (\mathbf{Y}, \mathbf{U}) \in \mathcal D_{Y,U}.  
\end{align}
where $ \left( \hat{\mathbf{X}}, \hat{\mathbf{Z}} \right) \in \mathcal D_{X,Z} \cap V $ are some fixed values for the complicating variables, and the set $V$  consists of those values of the complicating variables $\left( \mathbf{X}, \mathbf{Z} \right)$ for which the inner problem  $\mathcal{P}_{in}$ is feasible, i.e., $V = \{ \left( \mathbf{X}, \mathbf{Z} \right) :  \mathbf{G} \left( \mathbf{ X}, \mathbf{Z} , \mathbf{Y},\mathbf{U} \right) \geq 0\, ~ \text{for some}\, \left( \mathbf{Y}, \mathbf{U} \right) \in \mathcal D_{Y,U} \}$. 
%\begin{align}
%    V = \{ \left( \mathbf{X}, \mathbf{Z} \right) :  \mathbf{G} \left( \mathbf{ X}, \mathbf{Z} , \mathbf{Y},\mathbf{U} \right) \geq 0\, ~ \text{for some}\, \left( \mathbf{Y}, \mathbf{U} \right) \in \mathcal D_{Y,U} \}
%\end{align}
As such, $ \mathcal D_{X,Z} \cap V $ can be thought of as the projection of the feasible region of \eqref{eq: Porg_reformed} onto $\left( \mathbf{X}, \mathbf{Z} \right)$-space. %is the latest solution of the relaxed master problem.
%\blue{[NA: no need to mention this] Note that constraints \eqref{eq:capacity:storage} and \eqref{eq:const:delay2_e} which include only the complicating variables are not included in the inner problem and have been  moved directly to the outer problem.}
%!!!The inner problem is convex due to Lemma~\ref{lem:convex},

It can be easily verified that the inner problem is convex, and hence, can be solved in polynomial time using the conventional convex optimization approaches such as primal-dual interior point methods   \cite{boyd2009convex}.  Moreover, this problem is linearly separable in the simple and complicating variables. Therefore, it preserves Property P as well. %Consequently, the inner problem satisfies both conditions in Remarks 
Therefore, we can utilize GBD approach to efficiently solve the target optimization problem, as will be discussed in the rest of this section.


\iffalse ***

{\color{blue}{redundant to Lemma \ref{lem: slater}: (May be useful for somewhere else, I just keep it for now)  It can be easily verified that the inner problem is convex, and hence, can be solved in polynomial time, using the conventional convex optimization approaches (e.g., primal-dual interior point methods)  \cite{boyd2009convex}. 
\iffalse
\blue{{\color{red}{I have a Q here.}} Moreover, it can be verified that for any fixed %value of
$ \left( \mathbf{X} , \mathbf{Z} \right)  $, $ \left( \mathbf{Y}, \mathbf{U} \right) =\left( \mathbf{0}, \mathbf{\bar{U}} \right) $, where $\mathbf{\bar{U}} = \left\{u_{ns} = \dfrac{M_n}{(1- \alpha)|\mathbb S|D_s^{max}} , \forall n \in \{\mathbb E, c\}, \forall s \in \mathbb S\right\} $, is always a  feasible  solution to the inner problem. Therefore, the inner problem also satisfies Slater's condition.} 
\fi
Moreover, for any feasible %value of
$ \left( \mathbf{X} , \mathbf{Z} \right)  $, the inner problem includes only linear constraints, and hence, satifies Slater's condition.  Consequently, strong duality holds between $\mathcal P_{in}$ and its dual, and hence, the optimal %Lagrange 
multipliers associated with the constraints in $\mathcal P_{in}$ can be obtained % using the KKT conditions.   
(which are the Lagrangian multiplier vector) by using the primal-dual interior point methods. 
Finally, as discussed in the previous subsection, this problem is linearly separable in the simple and complicating variables, i.e., it preserves Property P. 
}}

*** 
\fi



At any iteration where the inner problem is feasible, let $\hat{\mathbf{ \mu}} \triangleq [\mathbf{\hat \mu}_{\ref{eq:sum1}}, \mathbf{\hat \mu}_{\ref{eq:capacity:bw}},  \mathbf{\hat \mu}_{\ref{eq:capacity:mu}}, \mathbf{\hat \mu}_{\ref{eq:stability:node}}, \mathbf{\hat \mu}_{\ref{eq:stability:link}} , \mathbf{\hat \mu}_{\ref{eq:const:delay2_a}} , \mathbf{\hat \mu}_{\ref{eq:const:delay2_b}} , \mathbf{\hat \mu}_{\ref{eq:const:delay2_c}} , \mathbf{\hat \mu}_{\ref{eq:const:delay2_d}} ]$ be the column vector of the  Lagrange multipliers of $\mathcal{P}_{in}$, whose entry $\mathbf{\hat \mu_{i}}, ~\forall i \in \{ \ref{eq:sum1} ,
\ref{eq:capacity:bw} , \ref{eq:capacity:mu}, \ref{eq:stability:node}, \ref{eq:stability:link} , \ref{eq:const:delay2_a},\ref{eq:const:delay2_b},\ref{eq:const:delay2_c},\ref{eq:const:delay2_d}  \} $ 
is the Lagrange multiplier vector associated with the constraints of the form $(i)$.
As such, for any fixed $\left( \mathbf{ X}, \mathbf{Z} \right)$, the upper-bounding function defined in \eqref{eq: L11} can be stated as
\begin{align} \label{eq: L upper star}
    L^*\left (\mathbf{X}, \mathbf{Z} ; \mathbf{\hat \mu} \right) = \max_{(\mathbf{Y}, \mathbf{U}) \in \mathcal D_{Y, U}}&~\mathcal R_{\text{srv}}({\mathbf{Y}}) - \mathcal P_{\text{cpu}}({\mathbf{U}}) -\mathcal P_{\text{trn}}({\mathbf{Y}}) \notag\\
    &+ \mathbf{\hat \mu}^T G(\mathbf{ X}, \mathbf{Z} , \mathbf{Y},\mathbf{U}) ,
\end{align}
%where $\mathbf{\hat \mu}$ is the optimal multiplier vector obtained in solving the inner problem $\mathcal{P}_{in}$. 

Regarding the optimization problem involved in the above upper-bounding function, first note that %under any fixed  $\left( \mathbf{\hat X}, \mathbf{\hat Z} \right)$ and 
{\color{red}{according to Property P, %(i.e., the linear separability property of the optimization problem in \eqref{eq: Porg_reformed}), 
the optimal solution to the above optimization equals to the optimal solution of the inner problem $\mathcal{P}_{in}$.}}  
%$(\mathbf{\hat Y}, \mathbf{\hat U})$ 
%\blue{[TO BE DONE LATER ON, if we have space: can be stated as a lemma. Lets keep it here for now.]} 
%Besides, due to complementary slackness property,  the inclusion of constraints including only the  continuous variables are not required in the above expression, as their associated terms in $\mathbf{\hat \mu}^T G(\mathbf{ X},\mathbf{Y},\mathbf{U})$ would be equal to zero.  
Second, %in \eqref{eq: L upper star} , 
according  to the complementary slackness property for the inner problem, those terms in $\mathbf{\hat \mu}^T G(\mathbf{ X},\mathbf{Y},\mathbf{U})$ associated with the constraints including only the continuous variables are equal to zero, and hence,  
 %we have only optimal Lagrange multipliers of
only the terms associated with constraints %of the form 
%\eqref{eq:routing} and 
\eqref{eq:const:delay2_a}--\eqref{eq:const:delay2_d} %\eqref{eq:const:delay2}  
are remained.   %\eqref{eq:p3:cons:sizing}. 
Therefore, if we let $\hat f$ denote the optimal value and $(\mathbf{\hat Y}, \mathbf{\hat U})$ denote the optimal solution of the inner problem, we have 
\begin{align} \label{eq: L super index star}
    L^* & \left(\mathbf{X}, \mathbf{Z}, \mathbf{\hat \mu} \right) =  \hat{f}\notag\\ 
    %& + \sum_{s \in \mathbb S}\sum_{e \in \mathbb E} \sum_{n \in \{ \mathbb E, c\}} \mu_{sen} (l_{en}x_{ns} - y_{sen}) \notag\\
    % + \mathbf{\hat \mu_{\ref{eq:routing}}}^T ~ [l_{en}x_{ns} - \hat y_{sen}, \forall s, e, n] \notag\\
    %& + \sum_{s \in \mathbb S}\sum_{e \in \mathbb E}  \omega_{es} (M_e x_{es} - u_{es}).
    %& + \mathbf{\hat \mu_{\ref{eq:p3:cons:sizing}}}^T [M_e x_{es} - \hat u_{es}, \forall s, e].
    %& + \mathbf{\hat \mu_{\ref{eq:delay}}}^T [ \blue{\cdots ,  \forall s, e, n}].
    &+ \mathbf{\hat \mu_{\ref{eq:const:delay2_a}}}^T ~ [  D^{\text{max}}_s (\hat u_{ns}/\nu_s - \hat \Lambda_{ns}) - z_{sen}, \forall s, e, n=e ] \notag \\
    &+ \mathbf{\hat \mu_{\ref{eq:const:delay2_b}}}^T ~ [  (1-\alpha) D^{\text{max}}_s (\hat u_{ns}/\nu_s - \hat \Lambda_{ns}) - z_{sen}, \forall s, e, n\neq e ] \notag \\
    &+ \mathbf{\hat \mu_{\ref{eq:const:delay2_c}}}^T ~ [  [\alpha D^{\text{max}}_s - d^{\text{prp}}_{en}]^+ (B^l_{en} - \hat \Lambda^l_{en}) - z_{sen},  \forall s, e, n \neq e ] \notag \\
    &+ \mathbf{\hat \mu_{\ref{eq:const:delay2_d}}}^T ~ [ z_{sen} - \hat y_{sen},  \forall s,e,n ].
\end{align}

Similarly, at any iteration where the inner problem is infeasible for the latest complicating variables $ \left( \hat{\mathbf{X}}, \hat{\mathbf{Z}} \right) $, the feasibility problem defined in \eqref{eq: L21} should be solved to obtain $\mathbf{\lambda}$ and consequently feasibility function. Due to Property P and inspired by \cite[Eq. (Q)]{zhang2015tuning}, we use an equivalent form of this problem as 
\begin{align}\label{eq: P_feas}
    \mathcal{P}_{feas}:
\quad&\min_{\mathbf{\alpha}, (\mathbf{Y}, \mathbf{U}) \in \mathcal D_{Y, U}} \alpha \notag\\
    \text{subject to}&\quad \mathbf{G} \left( \hat{\mathbf{X}}, \hat{\mathbf{Z}}, \mathbf{Y}, \mathbf{U} \right)+\mathbf{\alpha \underline{1}} \geq 0, 
\end{align}
where $\mathbf{\alpha}$ is a vector of the same size as the number of constraints. The above optimization problem can be easily solved  using convex optimization methods,
and its associated Lagrange multipliers compose the desired $\hat{\mathbf{\lambda}}$. We refer to the optimal solution of this problem as $(\bar{\mathbf{Y}}, \bar{\mathbf{U}})$ and define the feasibility function as
\begin{align}\label{eq: L subscript star}
    L_* & \left( \mathbf{X}, \mathbf{Z}  ; \mathbf{\hat \lambda} \right) = 
    %\sup_{(\mathbf{Y}, \mathbf{U}) \in \mathcal D_{Y, U}}  \left\{  {\mathbf{\hat \lambda}}^T \mathbf{G} \left( \mathbf{X} , \mathbf{Z},  \mathbf{Y}, \mathbf{U} \right)  \right\},
%  \end{align}
%  \begin{align}
    % &\mathbf{\hat \lambda_{\ref{eq:routing}}}^T ~ [l_{en}x_{ns} - \hat y_{sen}, \forall s, e, n] \notag\\
     \mathbf{\hat \lambda_{\ref{eq:const:delay2_a}}}^T ~ [ D^{\text{max}}_s (\bar u_{ns}/\nu_s - \bar \Lambda_{ns}) - z_{sen}, \forall s, e, n=e  ] \notag \\
    &+ \mathbf{\hat \lambda_{\ref{eq:const:delay2_b}}}^T ~ [ (1-\alpha) D^{\text{max}}_s (\bar u_{ns}/\nu_s - \bar \Lambda_{ns}) - z_{sen}, \forall s, e, n\neq e ] \notag \\
    &+ \mathbf{\hat \lambda_{\ref{eq:const:delay2_c}}}^T ~ [ [\alpha D^{\text{max}}_s - d^{\text{prp}}_{en}]^+ (B^l_{en} - \bar \Lambda_{en}) - z_{sen},  \forall s, e, n \neq e  ] \notag \\
    &+ \mathbf{\hat \lambda_{\ref{eq:const:delay2_d}}}^T ~ [ z_{sen} - \bar y_{sen},  \forall s,e,n  ].  
\end{align}

% where $\mathbf{\hat \lambda} \geq 0 $ is a  vector satisfying \cite{floudas1995nonlinear}

% \begin{align} \label{eq: lambda vector}
%     &\sup_{(\mathbf{Y}, \mathbf{U}) \in \mathcal D_{Y, U}}
%   \left\{  {\mathbf{\hat \lambda}}^T \mathbf{G} \left( \hat{\mathbf{X}}, \hat{\mathbf{Z}},\mathbf{Y},\mathbf{U} \right)  \right\} < 0, \notag \\
%     &\mathbf{1}^T \mathbf{\hat \lambda} = 1, 
% \end{align}

  
% Note that according to Property P, the optimization problem involved in  \eqref{eq: L subscript star} can be easily solved  using convex optimization methods, and its solution is obtained  independently of the value of the  complicating variables. 

%Finally, 
The current relaxed master problem can now be written as
\begin{subequations}\label{eq: P relaxed master}
\begin{align} 
\mathcal{P}_{out}^{{\text{relaxed}}}: 
&\max_{ \left( \mathbf{X} , \mathbf{Z} \right) \in \mathcal D_{X,Z}, \textsf{UB} \geq 0 }~\textsf{UB} - \mathcal P_{\text{str}}( \mathbf{X} )
\tag{\ref{eq: P relaxed master}} \\
    \text{subject to}\,\, ~ 
    &\eqref{eq:capacity:storage},\eqref{eq:const:delay2_e} \\ 
    &\mathsf{UB} \leq L^*\left (\mathbf{X},   \mathbf{Z} ;  \mathbf{\hat \mu}^{(j)} \right), ~ j=1,\ldots,\tau^{\text{feas}}, \label{eq: P relaxed master:L^*} \\ 
    &L_*\left (\mathbf{X},   \mathbf{Z} ;  \mathbf{\hat \lambda}^{(j)} \right) \geq 0, ~ j=1,\ldots,\tau^{\text{infeas}}.\label{eq: P relaxed master:L_*}
\end{align}
\end{subequations}
% The new constraint \eqref{eq:const:delay2_e} is added to guarantee that 
% the decided transfer variables by the master problem satisfy constraint \eqref{eq:routing} of the inner problem and to reduce the solution space. 
% Finally, according to the definition of the auxiliary variable $z_{sen}$, we should also have the following constraint
% \begin{equation}\label{eq:const:delay2_e}
%     z_{sen} \leq x_{ns}, ~ \forall s,e,n, 
% \end{equation}
% in order to guarantee that no requests for service $s$ arrived at $\mathrm{BS}_e$ can be transferred to server $n$ if it has not been placed in that server. 

The proposed algorithm can now be stated formally, which is represented by the following steps: 

\textbf{Step 1 (Initialization):} The algorithm starts with a feasible initial solution for the complicating variables, i.e., the service placement and request transfer variables. 
%!!!!that is feasible and also under which the inner problem remains feasible (i.e, there exists feasible solution for the simple variables, i.e., request admission and scheduling and CPU sizing variables). 

\textbf{Step 2 (Solving the Inner Problem):} For the fixed complicating variables, it uses the primal-dual interior-point method to solve the inner problem \eqref{eq: P_in} and find the optimal request scheduling and CPU sizing variables and the corresponding vector of Lagrange multipliers. 
As solution of the inner problem and the latest solution of the relaxed master problem maintain a lower-bound ($\mathsf{LB}$) and an upper-bound ($\mathsf{UB}$) to the solution of the original problem, respectively, one of the following three cases occurs:

%\textbf{Step 2A:} If the inner problem is feasible and the gap between its solution and the latest solution of the relaxed master problem (i.e., the upper-bound to the solution of the original problem) is still large, then the lower-bound $\mathsf{LB}$ will be recalculated and a new optimality cut in the form of  \eqref{eq: P relaxed master:L^*} is determined and added to the relaxed master problem. 
\textbf{Step 2A:} If the inner problem is feasible and the gap between its solution and the upper-bound is still large, then the lower-bound will be recalculated and a new optimality cut in the form of  \eqref{eq: P relaxed master:L^*} is determined and added to the relaxed master problem. 
%(i.e., the lower bound to the  solution of the original problem)

\textbf{Step 2B:} If the inner problem is infeasible, then the %infeasible 
violated constraints are identified using \eqref{eq: lambda vector}, and  a new feasibility cut in the form of \eqref{eq: P relaxed master:L_*} is determined and added to the relaxed master problem. 

\textbf{Step 2C:} If the inner problem is feasible and the gap between its solution and the upper-bound is small enough, then the algorithm stops and the latest solutions of the inner and relaxed master problems are returned as the output of the algorithm.

\textbf{Step 3 (Solving the Relaxed Master Problem):}
Having the new feasibility or optimality cuts added in Step~2 of the algorithm, the relaxed master problem is updated and solved \blue{[NA: Q] by any applicable algorithm} to realize a new solution for the service placement and service transfer variables, as well as a new upper-bound to the solution of the original problem. Then, the algorithm returns to Step 2.

The above steps are done iteratively until the gap between the lower and upper bounds becomes small enough. Finally, it outputs the optimal values of the service placement, service transfer, request scheduling, and CPU sizing variables. Algorithm~\eqref{alg:AO_method} presents the pseudo-code of the proposed algorithm.  
%These steps are summarized  [OR: the pseudo-code of the proposed method is presented ]  in Algorithm~\eqref{alg:AO_method}.

\begin{algorithm}[t]
\caption{ The proposed GBD-Based Algorithm.}
%to Optimize $\mathcal P_{org}$. 
\label{alg:AO_method}%\text{max\_iter\_num}
\begin{algorithmic}[1]
%!!! \State {\color{blue}{\textbf{Result:} Optimal $\mathbf{X}$, $\mathbf{Y}$, $\mathbf{U}$. }}
\State \textbf{Initialization:} Pick  $\left( \hat{\mathbf{X}} , \hat{\mathbf{Z}} \right) \in %{\color{red}{V \cap}}
\mathcal{D}_{X,Z}  $, and set  $\tau^{\text{feas}}=0$, $\tau^{\text{infeas}}=0$, $\textsf{UB}= + \infty$, $\textsf{LB}= - \infty $, and the convergence tolerance parameter $\epsilon \geq 0$.

%\MA{I think we can just initialize without definition}\blue{[the counter for the number of feasible iterations $\tau^{\text{feas}}= %1
%0$, the counter for the number of infeasible iterations $\tau^{\text{infeas}}=0$, the counter for the total number of iterations $\tau =1 $, the convergence tolerance parameter $\epsilon >0$,  the maximum number of iterations $ \tau^{\text{max}} \in \mathbb{N}$, and the upper and lower bounds $\textsf{UB}= + \infty %2 \epsilon 
%$ and $\textsf{LB}= - \infty $, respectively.]}

%!!!! \State {\color{red}{Determine a vector}} $ \mathbf{\lambda}^0 \geq \mathbf{0} $ satisfying \eqref{eq: lambda vector}. 

\iffalse 
\State {\color{red}{Solve the inner  problem}}  $\mathcal{P}_{in}$ in \eqref{eq: P_in} for $\left( \hat{\mathbf{X}} , \hat{\mathbf{Z}} \right)$, using primal-dual interior point method, %by any convex optimization method,  
and obtain its optimal value  $F\left( \hat{\mathbf{X}} , \hat{\mathbf{Z}} \right)$, its optimal solution $\left( \hat{\mathbf{Y}},\hat{\mathbf{U}} \right)$ and the corresponding Lagrange  multipliers vector $\mathbf{\hat \mu}^{\tau^{\text{feas}}}$.
\fi

%\While{$\textsf{UB} - \textsf{LB} > \epsilon$ and $\tau < \tau_{\text{max}}$}

\iffalse
\State {\color{blue}{$\textsf{LB} \leftarrow \max \{\textsf{LB},  F\left( \hat{\mathbf{X}} , \hat{\mathbf{Z}} \right)\}$.}}

%\For{$j\in [1:\text{max\_iter\_num}]$}

\State Solve the  current relaxed master problem  defined by \eqref{eq: P relaxed master}, 
\blue{by any applicable algorithm}, and obtain its optimal solution $ \left( \hat{x}_0, \hat{\mathbf{X}} , \hat{\mathbf{Z}} \right) $. \label{alg:master}

\State {\color{blue}{$\mathsf{UB}  \leftarrow  \hat{x}_0 $.}}

\If{$ \mathsf{UB} - \mathsf{LB} \leq \epsilon $}
\State Go to Line \ref{alg:output}. %!!!! Terminate.
\EndIf

\fi

\State \textbf{Inner problem:} Solve the inner problem $\mathcal{P}_{in}$ in \eqref{eq: P_in} for $\left( \hat{\mathbf{X}} , \hat{\mathbf{Z}} \right)$, %!!!! by any convex optimization method, 
by the primal-dual interior point method, 
and obtain (if exist) its optimal value  $f\left( \hat{\mathbf{X}} , \hat{\mathbf{Z}} \right)$, its optimal solution $\left( \hat{\mathbf{Y}},\hat{\mathbf{U}} \right)$ and the corresponding Lagrange  multipliers vector $\mathbf{\hat \mu}$. \label{alg:inner}
%and obtain (if they  exist)  $\left( \hat{\mathbf{Y}},\hat{\mathbf{U}} \right)$, $F\left( \hat{\mathbf{X}} , \hat{\mathbf{Z}} \right)$, and the corresponding Lagrangian dual multipliers vector $\mathbf{\hat \mu}^{\tau^{\text{feas}}}$.

\If{$ - \infty < f\left( \hat{\mathbf{X}} , \hat{\mathbf{Z}} \right) < \mathsf{UB} - \epsilon $ }

%\State{\If{ddd}
%\State{jjj}
%\EndIf
%}

\State $ \tau^{\text{feas}} \leftarrow \tau^{\text{feas}} +1$.
\State $\mathbf{\hat \mu}^{\tau^{\text{feas}}} \leftarrow \mathbf{\hat \mu} $
\State $\textsf{LB} \leftarrow \max \{\textsf{LB},  f\left( \hat{\mathbf{X}} , \hat{\mathbf{Z}} \right)\}$.
\EndIf

\If{$ f\left( \hat{\mathbf{X}} , \hat{\mathbf{Z}} \right) = - \infty $} %(i.e., the inner problem is infeasible)


\State $ \tau^{\text{infeas}} \leftarrow \tau^{\text{infeas}} +1$.
%\State{$ \lambda^q \leftarrow \mathbf{\hat{\lambda}} $}.

\State Solve the feasibility problem $\mathcal{P}_{feas}$ in \eqref{eq: P_feas} for $\left( \hat{\mathbf{X}} , \hat{\mathbf{Z}} \right)$, and obtain its optimal solution $\left( \bar{\mathbf{Y}},\bar{\mathbf{U}} \right)$ and the corresponding Lagrange  multipliers vector $ \mathbf{\lambda}^{\tau^{\text{infeas}}}$.
%Determine a vector $ \mathbf{\lambda}^{\tau^{\text{infeas}}} \geq \mathbf{0} $ satisfying \eqref{eq: lambda vector}. 

\EndIf

\If{
%$ \mathsf{UB} - \mathsf{LB} \leq \epsilon$ 
$ \mathsf{UB} - \epsilon \leq f\left( \hat{\mathbf{X}} , \hat{\mathbf{Z}} \right) < \infty $}
%\If{$ \mathsf{UB} - \epsilon \leq F\left( \hat{\mathbf{X}} , \hat{\mathbf{Z}} \right) < \infty $ }
\State Go to Line \ref{alg:output}. %!!!!{Terminate.}

\EndIf


\iffalse\State{ Go to Line~\ref{alg:master}.}
\fi

\State \textbf{Outer problem:} Solve the  current relaxed master problem  defined by \eqref{eq: P relaxed master}, 
\blue{[NA: Q] by any applicable algorithm}, and obtain its optimal solution $ \left( %!!!!\hat{x}_0
\mathsf{UB}, \hat{\mathbf{X}} , \hat{\mathbf{Z}} \right) $. \label{alg:master}

%!!!!\State {\color{blue}{$\mathsf{UB}  \leftarrow  \hat{x}_0 $.}}

%\ElseIf{$ \mathsf{LB} <  F\left( \hat{\mathbf{X}} , \hat{\mathbf{Z}} \right) < \infty $}

%\Elsif{ddd}


%\State $\tau \leftarrow \tau +1$.
%\EndWhile

\State Return to Line \ref{alg:inner}.

\State {\textbf{Output:}} $ \left( \mathbf{X}^\ast , \mathbf{Z}^\ast, \mathbf{Y}^\ast , \mathbf{U}^\ast \right) \leftarrow \left( \hat{\mathbf{X}} ,  \hat{\mathbf{Z}} , \hat{\mathbf{Y}}, \hat{\mathbf{U}} \right) $. \label{alg:output}
% \If{$LBD \geq y_0 - \epsilon$}
% \State Return $\left(  \hat{\mathbf{X}},\hat{\mathbf{Z}},\hat{\mathbf{Y}},\hat{\mathbf{U}} \right)$. 
% \State Terminate.
% \EndIf
%\EndFor
\end{algorithmic}
\end{algorithm}



A few remarks regarding the proposed algorithm are in place. \NA{In case it is needed to add some points regarding the algorithm, we will discuss them here:}

\begin{remark}[\textbf{Complexity of the Inner and Outer Problems}]

    Note that solving the inner and the relaxed master problems in the proposed algorithm are much easier than solving the original problem. 
    This is due to the fact that for fixed values of the complicating variables $\left( \mathbf{X},\mathbf{Z} \right)$, problem $\mathcal{P}_{in}$ is a convex optimization problem, and hence, can be solved in polynomial time by using the conventional convex optimization approaches (e.g., primal-dual interior point methods) \cite{boyd2009convex}. Moreover, it is noted that using primal-dual interior point methods, the optimal Lagrange multipliers corresponding to the inner problem can also be achieved simultaneously, which will be used in the algorithm as well.
    In addition, regarding the relaxed master problem \eqref{eq: P relaxed master}, %the objective function is clearly linear and 
    the optimizations involved in determining the Lagrange functions $L^\ast$ and $L_\ast$ are also convex optimization problems. This is  due to the fact that their objective functions are linearly separable in the binary and real variables, and hence, these problems preserve Property P which allows to %obtain an explicit form for the aforementioned functions, and hence, 
    take the involved supremums over $\mathcal D_{Y,U}$ independently of the binary variables $\left( \mathbf{X} , \mathbf{Z} \right)$. As such, the relaxed master problem \eqref{eq: P relaxed master} is no longer an MINLP, but just an ILP that can be solved efficiently via the existing efficient approaches \blue{(e.g., see [ref??])}. 
    
\end{remark}
\MA{In general, this section has many similarities with the previous paragraphs, I will revise it at the end of work. maybe only keeping Remark and putting details in the algorithm itself.}
\section{Convergence Analysis}
%and possible enhancements

In this section, we present theoretical  convergence results of the proposed algorithm. In particular, we prove the proposed algorithm converges to a stationary point of the original problem in a finite number of iterations. For this purpose, we first state and prove the following lemmas.

\begin{lemma}\label{lem: lem1_alternative}
    The set $\mathcal D_{Y,U}$ is non-empty, convex, bounded and closed. 
\end{lemma}

\begin{proof}
 The proof follows a direct result of the definition of the set $\mathcal D_{Y,U}$. (\blue{OR: [Which one do you prefer? the first one.]} the statement of the lemma is clear, due to the definition of the set $\mathcal D_{Y,U}$.)
\end{proof}

\begin{lemma}
    The constraint functions in $ \mathbf{G} \left( \mathbf{X} , \mathbf{Z} ,\mathbf{Y},\mathbf{U} \right) $ are concave and continuous on $\mathcal D_{Y,U}$, for any fixed $\left( \mathbf{X} , \mathbf{Z} \right) \in \mathcal D_{X,Z} $.
\end{lemma}

\begin{proof}
    For any fixed value of $\left( \mathbf{X} , \mathbf{Z} \right) \in \mathcal D_{X,Z} $, all the constraint functions in $ \mathbf{G} \left( \mathbf{X} , \mathbf{Z} ,\mathbf{Y},\mathbf{U} \right) $ are linear over $\left( \mathbf{Y},\mathbf{U} \right)$ and hence, also concave. Moreover, due to \ref{lem: lem1_alternative} and the linearity of the constraint functions in $ \mathbf{G} \left( \mathbf{X} , \mathbf{Z} ,\mathbf{Y},\mathbf{U} \right) $, these functions are also continuous on $D_{Y,U}$, for each fixed $ \left( \mathbf{X} , \mathbf{Z} \right) \in \mathcal{D}_{X,Z} $. 
\end{proof}

\iffalse
\begin{lemma}\label{lem: lem1}
    $\mathcal D_{Y,U}$ is a non-empty convex set, and the constraint functions in $ \mathbf{G} \left( \mathbf{X} , \mathbf{Z} ,\mathbf{Y},\mathbf{U} \right) $ are concave on $\mathcal D_{Y,U}$ for any fixed $\left( \mathbf{X} , \mathbf{Z} \right) \in \mathcal D_{X,Z} $.
\end{lemma}

\begin{proof}
    The first statement is clear, due to the definition of the set $\mathcal D_{Y,U}$. 
    Moreover, since for any fixed value of $\left( \mathbf{X} , \mathbf{Z} \right) \in \mathcal D_{X,Z} $, all the constraint functions in $ \mathbf{G} \left( \mathbf{X} , \mathbf{Z} ,\mathbf{Y},\mathbf{U} \right) $ are linear over $\left( \mathbf{Y},\mathbf{U} \right)$, it is also concave. 
\end{proof}

\begin{lemma}
For each fixed $ \left( \mathbf{X} , \mathbf{Z} \right) \in \mathcal{D}_{X,Z} $, the set 
\begin{align}
    &S_{X,Z} \triangleq  \\
    &\left\{ \mathbf{s} \in \mathbb{R}^m: \mathbf{G} \left( \mathbf{X} , \mathbf{Z} ,\mathbf{Y},\mathbf{U} \right) \geq \mathbf{s},  \mathrm{~for~some~} \left( \mathbf{Y},\mathbf{U} \right) \in \mathcal D_{Y,U} \right\}, \notag
\end{align}
where $m$ is the number of constraints involved in the inner problem $\mathcal{P}_{in}$ (i.e., the constraints 
%\eqref{eq:sum1}--\eqref{eq:capacity:mu},  \eqref{eq:stability:node}--\eqref{eq:stability:link}, %\blue{and \eqref{eq:delay}}. 
\eqref{eq:sum1}, \eqref{eq:capacity:bw}, \eqref{eq:capacity:mu}, \eqref{eq:stability:node}, \eqref{eq:stability:link}, 
and \eqref{eq:const:delay2_a}--\eqref{eq:const:delay2_d}\footnote{ %which can be identified as 
It can be identified that $m=4SE \left(E+1\right) + E^2 +E+S$. \MA{$m=4SE \left(E+1\right) + E^2 +2E+S(E+1)$.}}) 
is closed.

\MA{I added constraint \eqref{eq:const:delay2_e} to the master which reduces the solution space and guarantees \eqref{eq:routing}. Thus, \eqref{eq:routing} can be removed from the inner as noted in the first paragraph of V-C. In this way $m=3SE \left(E+1\right)+E^2+2E+S(E+1).$}
\end{lemma}

\begin{proof}
First note that it can be verified that for each $\mathbf{s}_0 \in S_{X,Z}$, all the points $\mathbf{s} \preccurlyeq \mathbf{s}_0 $ also belongs to $S_{X,Z}$. 
 Moreover, for each $i=1,\cdots,m$, $\mathbf{G}^{(i)}  \left( \mathbf{X} , \mathbf{Z} ,\mathbf{Y},\mathbf{U} \right)$  which is the $i^\mathrm{th}$ element in $\mathbf{G} \left( \mathbf{X} , \mathbf{Z} ,\mathbf{Y},\mathbf{U} \right)$ is determined by one of the constraints defined in \eqref{eq:sum1}, \eqref{eq:capacity:bw}, \eqref{eq:capacity:mu}, \eqref{eq:stability:node}, \eqref{eq:stability:link}, 
and \eqref{eq:const:delay2_a}--\eqref{eq:const:delay2_d}, which are all affine. % constraints.
For each $i=1,\cdots,m$,  define the following set
\begin{align}
    &S_{X,Z}^{(i)} \triangleq  \\
    &\left\{ s \in \mathbb{R}: \mathbf{G}^{(i)} \left( \mathbf{X} , \mathbf{Z} ,\mathbf{Y},\mathbf{U} \right) \geq s,  \mathrm{~for~some~} \left( \mathbf{Y},\mathbf{U} \right) \in \mathcal D_{Y,U} \right\}, \notag
\end{align}






As such, it can be verified that for each $i=1,\cdots,m$, $s_i$ which is the $i^\mathrm{th}$ element of $\mathbf{s}$,  belongs to the set of half-space determined by the associated affine  constraint.  Therefore, the vector 

    For each fixed $ \left( \mathbf{X} , \mathbf{Z} \right) \in \mathcal{D}_{X,Z} $, the set $S_{X,Z}$ can be rewritten as
    \begin{align}
        & S_{X,Z} \notag   \\
    & = \left\{ \mathbf{s} \in \mathbb{R}^m: \mathbf{G} \left( \mathbf{X} , \mathbf{Z} ,\mathbf{Y},\mathbf{U} \right) \geq \mathbf{s},  \mathrm{~for~some~} \left( \mathbf{Y},\mathbf{U} \right) \in \mathcal D_{Y,U} \right\}, \notag \\ 
    & = \left\{ \mathbf{s} \in \mathbb{R}^m: - \mathbf{s} \geq - \mathbf{G} \left( \mathbf{X} , \mathbf{Z} ,\mathbf{Y},\mathbf{U} \right),   \mathrm{~for~some~} \left( \mathbf{Y},\mathbf{U} \right) \in \mathcal D_{Y,U} \right\}, \notag \\
    & = - epi -  \mathbf{G} \left( \mathbf{X} , \mathbf{Z} ,\mathbf{Y},\mathbf{U} \right),
    \end{align}
    
    
\end{proof}

%The following Lemma (which is similar to the lemma in Paper: A_Benders_Decomposition_Approach_for_Resilient_Placement_of_Virtual_Process_Control_Functions_in_Mobile_Edge_Clouds.pdf) is the substitute for its next lemma

\begin{lemma}
$D_{Y,U}$ is bounded and closed, and the constraint functions in $ \mathbf{G} \left( \mathbf{X} , \mathbf{Z} ,\mathbf{Y},\mathbf{U} \right) $
are continuous %on the domain of Y,U
on $D_{Y,U}$ for each fixed $ \left( \mathbf{X} , \mathbf{Z} \right) \in \mathcal{D}_{X,Z} $. 
\end{lemma}

\begin{proof}
 The first statement is clear, due to the definition of the set $\mathcal D_{Y,U}$, and hence due to the linearity of the constraint functions in $ \mathbf{G} \left( \mathbf{X} , \mathbf{Z} ,\mathbf{Y},\mathbf{U} \right) $, these functions are continuous on $D_{Y,U}$ for each fixed $ \left( \mathbf{X} , \mathbf{Z} \right) \in \mathcal{D}_{X,Z} $. 
\end{proof}
\fi

\begin{lemma}\label{lem: strong duality}
Strong duality holds for the  inner problem $\mathcal{P}_{in}$. %is convex and satisfies Slater's condition. 


\end{lemma}\label{lem: slater}

\begin{proof}
It can be easily verified that the inner problem $\mathcal{P}_{in}$ in \eqref{eq: P_in} is convex. 
Furthermore, since for any feasible %value of
$ \left( \mathbf{X} , \mathbf{Z} \right)  $, the inner problem includes only linear constraints, it  satisfies Slater's condition too.  Consequently, strong duality holds between $\mathcal P_{in}$ and its dual. 
\end{proof}

\begin{lemma}\label{lem: opt multplr vec}
%For any fixed $\left( \mathbf{X} , \mathbf{Z} \right) \in \mathcal D_{X,Z} $, $f \left( \hat{\mathbf{X}} , \hat{\mathbf{Z}}  \right) = + \infty$ , or $f \left( \hat{\mathbf{X}} , \hat{\mathbf{Z}}  \right) $ is finite and the inner problem possesses an optimal multiplier vector.

For any fixed $\left( \mathbf{X} , \mathbf{Z} \right) \in \mathcal D_{X,Z} \cap V $, the solution of the inner problem $\mathcal{P}_{in}$ % in \eqref{eq: P_in} 
  is either unbounded or bounded %(i.e., $f \left( \mathbf{X} , \mathbf{Z}  \right)$ in \eqref{eq: P_in}  is finite) 
  with the inner problem possessing an optimal multiplier vector.
%37~ Y c~ V, at least one of the follow- ing three conditions holds: (a) v(37) is finite and ( l - j ) possesses an optimal multiplier vector, or (b) $v(j) = +\infty$.
\end{lemma}

\begin{proof}
First, note that according to the definition of $V$, for any $\left( \mathbf{X} , \mathbf{Z} \right) \in \mathcal D_{X,Z} \cap V $, the problem $\mathcal{P}_{in}$ never gets infeasible. Therefore, either $f \left( \mathbf{X} , \mathbf{Z}  \right) = + \infty $ or $f \left( \mathbf{X} , \mathbf{Z}  \right) $ is finite. In the latter case, since according to Lemma \ref{lem: strong duality}, strong duality holds between  problem $\mathcal{P}_{in} $ and its dual,  
%and hence, optimal multipliers exist for this problem which are the solution to the dual problem.
this problem possesses an optimal %Lagrange 
multiplier vector  which is the Lagrangian multiplier vector   associated with the constraints in $\mathcal P_{in}$ (which is the solution to the dual problem) and is obtainable % using the KKT conditions. 
via the primal-dual interior point methods. 

%... {\color{red}{(I have a Q here, asked on Whatsapp)}}


%{\color{blue}{(Perhaps, no need here:) Finally, as discussed in the previous subsection, this problem is linearly separable in the simple and complicating variables, i.e., it preserves Property P.}}  

\end{proof}

\begin{theorem}[Finite Convergence]
 The proposed GBD-based procedure in Algorithm  \ref{alg:AO_method}  terminates in a finite number of steps for any given $\epsilon \geq 0$. 
\end{theorem}

\begin{proof}
%Since the RVP algorithm satisfies conditions 1) to 5), by [30, Th. 6.4.3] it terminates in a finite number of iterations for any ε>0.

According to Lemmas \ref{lem: lem1_alternative}--\ref{lem: opt multplr vec} and \cite{floudas1995nonlinear}[Theorem 6.3.4], \blue{[NA: I have a Q here] the proposed GBD-based algorithm (OR: Algorithm \ref{alg:AO_method})} terminates in a finite number of iterations for any given $\epsilon \geq 0$. 
% The proof follows a direct result of Lemmas \ref{lem: lem1_alternative}--\ref{lem: opt multplr vec} and \cite{geoffrion1972generalized}[Theorem 2.4]. 
\end{proof}

%
%\blue{------------------------------------------------------}
%
%\NA{--------OLD VERSION from here till the end: ----
%(I am using some parts and will remove them entirely afterwards.)}

%{\color{gray}{
%Outer problem is
%\begin{align}  \label{eq: P_out}
%\mathcal{P}_{out}: 
%&\max_{ \mathbf{X} ,  \mathbf{Z} } ~ 
%F  \left( \mathbf{X},\mathbf{Z} \right)
%\notag \\
%    \text{subject to}\,\, & %\notag \\
%    %& \left( \mathbf{X} , \mathbf{Z} \right) \in V, \notag \\
%    (1), (3), (5), (8), \notag \\
%    &\left(\mathbf{X},\mathbf{Z}\right) \in V \cap \mathcal D_{X,Z},
%\end{align}
%where 
%\begin{align} \label{eq: set V}
% V \triangleq \{  
%\left( \mathbf{X} , \mathbf{Z} \right):  ~ \mathbf{G} &\left( \mathbf{X},\mathbf{Z},\mathbf{Y},\mathbf{U} \right) \geq 0 \quad  \notag \\
%&\text{for some}  \left(\mathbf{Y},\mathbf{U} \right) % \in  \mathcal D_{Y,U} 
%\text{feasible in}  ~ \mathcal{P}_{in}
%%{\color{blue}{(/for some feasible point in P_in)}}
%\}, 
%\end{align} %In fact, the set $V$
%consists of  those values of $\left( \mathbf{X} , \mathbf{Z} \right)$ for which the inner problem $\mathcal{P}_{in}$ remains  feasible. 
% Note that under the above decomposition, the inner problem optimizes the real variables for some  fixed values of  the complicating (i.e., the integer) variables $\mathbf{X} , \mathbf{Z} $. %Moreover, 
%It should also be noted that %by the above decomposition, 
%the outer problem $\mathcal{P}_{out}$ is %!!!!in fact, 
%the projection of the original problem $\mathcal{P}_{org}$ onto $\left( \mathbf{X} , \mathbf{Z} \right)$. In fact, the concept of projection [ref?] enables the original problem to be viewed as a problem in $\left( \mathbf{X} , \mathbf{Z} \right)$-space. % [ref?]. 
%Note that due to the primal decomposition, the projected problem $\mathcal{P}_{out}$ is equivalent to the original problem $\mathcal{P}_{org}$  \cite{palomar2006tutorial}, \cite{bertsekas1997nonlinear}.
%
%%In the rest of this section, we discuss how to handle the outer and inner problems. For this purpose, first note that evaluating $ F \left( \mathbf{X},\mathbf{Z} \right) $ in the inner problem is much easier than solving the original problem. This is due to the fact that for fixed values of the complicating variables $\left( \mathbf{X},\mathbf{Z} \right)$, problem $\mathcal{P}_{in}$ is a convex optimization problem, and hence, can be solved in polynomial time by using the existing/conventional convex optimization approaches (e.g., primal-dual interior point methods) \cite{boyd2009convex}.
%%However, the outer problem %is still an MINLP problem. 
%%still includes some challenges that need to be addressed properly: First, it is an MINLP problem. Second, the function $ F \left( \mathbf{X},\mathbf{Z} \right) $ and the set $V$ are only known implicitly via their definitions \eqref{eq: P_in} and \eqref{eq: set V}. To address the aforementioned challenges, we utilize the generalized Benders decomposition (GBD) approach, as will be illustrated in the next subsection.
%}}

